The Sub-mm Variability of IRC+10216 and $o$ Ceti

We present the sub-mm variability of two of the most well studied AGB stars, IRC+10216 and $o$ Ceti. The data are obtained at $450~\micron$ and $850~\micron$ as part of pointing calibration observations for the James Clerk Maxwell Telescope's SCUBA-2 instrument over a span of 7 years. The periods are derived using non-parametric methods, \texttt{Gatspy Supersmoother} and \texttt{P4J} in order not to assume an underlying shape to the periodicity. These were compared to two Lomb-Scargle parametric methods. We find that for both sources and wavelengths the periods derived from all methods are consistent within $1\sigma$. The $850~\micron$ phase folded light curves of IRC+10216 show a time lag of $\sim 540$ days compared to its optical counterpart. We explore the origins of the sub-mm variability and the phase lag using radiative transfer models. Combining the modelling with findings in the literature, we find that the sub-mm emission and phase lag can be partially attributed to the dust formation/destruction cycle. A second, unknown mechanism must be invoked; we defer an investigation of the origin and nature of this mechanism to a future work.

==> Tables/PublishedPeriods_CWLeo.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}
  \centering
  \caption{Periods Reported in Literature for IRC+10216 and \textit{o} Ceti}
    \begin{tabular}{llll}
    
    \hline
    \hline
    
    Wavelength & Telescope/Instrument & Period (Days) & Reference \\
    
    \hline

IRC+10216 &&\\

    Radio continuum - 8.4, 14.9 and 22.5 GHz & NRAO Very Large Array & $535 \pm 51$ & \citet{Menten2006_CWLeoRadio} \\
    
    Sub-mm continuum - 250, 350 and 450 $\micron$ & Herschel/SPIRE &  & $639 \pm 4$  & \citet{Groenewegen2012IRC+10216} \\
    
    Optical & Various & $630 - 650$ &  \citet{Witteborn1980-CWLeoVariability}, \\
    &&& \citet{Dyck1991-CWLeoVariability}, \\ 
    &&& \citet{LeBertre1992-CstarLightCurves}  \\

    
    \hline
    \hline
    
    \end{tabular}%
  \label{Table:PublishedPeriods_CWLeo}%
\end{table*}%



The period determined by \citet{Groenewegen2012IRC+10216} is similar to optical measurements that lie within a period range of $630-650$ days \citep{Witteborn1980-CWLeoVariability, Dyck1991-CWLeoVariability, LeBertre1992-CstarLightCurves}. \citet{Dehaes2007} determine a period of 655.3 days using 1.2 mm continuum observations. Molecular line observations by \citet{Teyssier2015-CWLeoMolecularLines} using Herschel HIFI, SPIRE, and PACS show periods between $\sim 600-760$ days for the HCN in the circumstellar envelope of IRC+10216. \citet{Kim2015-CWLeoVariability} derived a period of $640 \pm 0.9$ days in the optical using data from \citet{Drake2014-CatlinaSurvey}. Similarly they derived periods in the JHKLM bands using light curve data from \citet{LeBertre1992-CstarLightCurves} and \citet{Shenavrin2011-StellarVariability}. The derived periods for the two data sets are $627 \pm 26$ and $633 \pm 6 $.  These published results are summarised in table XX. 
























==> Tables/Sec_Periods_CWLeo.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}
  \centering
  \caption{Secondary Peak Periods of IRC+10216 $450~\micron$}
    \begin{tabular}{ll}
    \hline
    \hline
    \multirow{2}[0]{*}{Period Method} & \multirow{1}[0]{*}{$450~\micron$ Secondary}
   
    \\
   
   &  Peak Period (days) 
   
    \\
    \hline

    Astropy LombScargle   & $661$ \\

    Gatspy SlowLomb    & $665$  \\

    \hline
    \hline
    \end{tabular}%
   \label{Table:Secondary_Periods}
\end{table}%
